"It makes you think": Provocations Help Restore Critical Thinking to AI-Assisted Knowledge Work

Recent research suggests that the use of Generative AI tools may result in diminished critical thinking during knowledge work. We study the effect on knowledge work of provocations: brief textual prompts that offer critiques for and propose alternatives to AI suggestions. We conduct a between-subjects study (n=24) in which participants completed AI-assisted shortlisting tasks with and without provocations. We find that provocations can induce critical and metacognitive thinking. We derive five dimensions that impact the user experience of provocations: task urgency, task importance, user expertise, provocation actionability, and user responsibility. We connect our findings to related work on design frictions, microboundaries, and distributed cognition. We draw design implications for critical thinking interventions in AI-assisted knowledge work.

==> AccessibilityDescriptions.tex <==
Figure 1: "A schematic overview of the shortlisting interface. The first part of the overview shows Step 1: Enter shortlist objective -- below is a basic spreadsheet on the left with 3 columns (Name, Amount, Description). To the right of this spreadsheet is an input text-field with the text 'Shortlist charities that prioritise children'. There is a mouse cursor hitting a submit arrow. To the right of Step 1 is Step 2: Shortlisting factors generated -- this step shows 2 versions of the system: Step 2a: Without provocations -- shows a similar interface to Step 1 but under the input text-field is 4 factor cards organized in a 2x2 grid with factor titles of Target group, Grant amount, Specificity, and Geo reach. In each factor card is a green 'Apply' button. The mouse cursor now hovers over the Apply button of Grant amount. Under Step 2a is Step 2b With provocations -- This is the same interface as Step 2a but has provocations as a yellow text box in each factor card saying 'Consider...'. Finally, to the right of Step 2 there is Step 3 Applying factors creates shortlist -- this shows the same interface but with the spreadsheet highlighting the top 3 rows in green representing a sorted and highlighted shortlist."
 
Figure 2: "Detailed view of the factor cards presented in Figure 1. On the left half of the figure, a title of 'Factor card without provocations' is above a factor card. The factor card is a grey box. At the top is the factor title 'Target population mention'. Under this is a label 'Column(s)' next to a drop-down UI element with 'Description' selected. Next to the drop-down is a plus sign representing the ability to add new columns to the factor card. Below this is the label 'Criteria' which is above a text-area containing the sentence 'Contains keywords such as children, youth, families, young people. Below this text-area is a label of 'Importance', next to 3 radio buttons of Low, Medium, and High, with High being selected. Finally, A green 'Apply' button sits at the bottom of the card. To the right half of the figure, a title of 'Factor card with provocations' is above a factor card. This factor card is the same as the card on the left, except between the 'Importance' section and the 'Apply' button is the provocation text highlighted in yellow, saying 'May exclude grants that benefit children indirectly. Consider also looking for terms like education, school, playground, childcare. Finally, to the right of this factor card is a list of the different parts of a factor card from top to bottom: A. Factor Title, B. Target columns, C. Factor Criteria prompt (user editable), D. Importance weighting, E. Provocation."

Figure 3: "Two kernel density estimate plots the two datasets, Charity Dataset on the left half of the figure, and Movies Dataset on the right. On the y-axis is the density measure and on the x-axis of both plots is the Similarity Rating for the Rank-Biased Overlap (or RBO). On the left Charity Dataset plot, in red, is the KDE plot for Provocations, peaking between 0.0 and 0.5 RBO with a red dotted median line at 0.3023, and in blue is the KDE plot for No Provocations peaking near 0.5 with a blue dotted median line at 0.4683. The right Movies dataset plot, in red, is the Provocations KDE plot peaking a little passed 0.5, and a red dotted median line at 0.5533, and in blue is the KDE plot for No Provocations peaking between 0.5 and 1.0 RBO with a blue dotted median line at 0.7645."

Figure 4: "Histograms of the count of Think Aloud and System Action codes. On the left histogram is the count of think aloud codes. Each code has 2 bars, the blue bar on the left representing count of No Provocation occurrences for the code, and the orange bar on the right of Provocation counts. The X axis is each code (TA-CONS, TA-CRIT, TA-FACT, TA-FLSL, TA-GBSL, and TA-IMP, which are described in Table 1). The Y-axis is the count of the code occurrences. Each Code is displayed as such: TA-CONS - No Provocations bar near 50, Provocations bar near 70. TA-CRIT - No Provocations bar near 35, Provocations bar near 45. TA-FACT - No Provocations bar near 55, Provocations bar near 65. TA-FLSL - No Provocations bar near 10, Provocations bar near 20. TA-GBSL - No Provocations bar near 55, Provocations bar near 60. TA-IMP - No Provocations bar near 45, Provocations bar near 40.
On the right histogram is the count of action codes. Each code has 2 bars, the blue bar on the left representing count of No Provocation occurrences for the code, and the orange bar on the right of Provocation counts. The X axis is each code (A-ADDF, A-AFAC, A-ECRIT, A-EIMP, and A-VGSL, which are described in Table 1). The Y-axis is the count of the code occurrences. Each Code is displayed as such: A-ADDF - No Provocations bar near 4, Provocations bar near 2. A-AFAC - No Provocations bar near 55, Provocations bar near 55. A-ECRIT - No Provocations bar near 25, Provocations bar near 25. A-EIMP - No Provocations bar near 15, Provocations bar near 20. A-VGSL - No Provocations bar near 55, Provocations bar near 55."

Figure 5: "Three horizontal stacked-bar plots of the results of the three provocation evaluation questionnaires. At the top is Plot A titled 'Provocations were helpful in.' 3 bars are present, with the label on the left part of the Y-axis. 
The 1st bar 'Thinking about the shortlist factors' has 1 for Neutral, 3 for Agree, and 8 for Strongly Agree. 
The 2nd bar 'Evaluating the temporary shortlist' has 1 for Neutral, 8 for Agree, and 3 for Strongly Agree. 
The 3rd bar 'Finalizing the shortlist has 1 for Disagree, 3 for Neutral, 4 for Agree, and 4 for Strongly Agree.
Under this is plot B. A horizontal stacked-bar plot titled 'The provocations I saw.' 7 bars are present, with the label on the left part of the Y-axis. 
The 1st bar 'Influenced my decisions' has 2 for Disagree, 1 for Neutral, 5 for Agree, and 4 for Strongly Agree. 
The 2nd bar 'Provided enough info to make a decision' has 3 for Disagree, 3 for Neutral, 4 for Agree, and 2 for Strongly Agree. 
The 3rd bar 'Were actionable' has 5 for Neutral, 6 for Agree, and 1 for Strongly Agree. 
The 4th bar 'Were relevant to my preference' has 1 for Strongly Disagree, 3 for Neutral, 4 for Agree, and 4 for Strongly Agree. 
The 5th bar 'Were relevant to the factor' has 2 for Neutral, 4 for Agree, and 6 for Strongly Agree. 
The 6th bar 'Were useful in helping me critically think about my problem' has 2 for Disagree, 2 for Neutral, 4 for Agree, and 4 for Strongly Agree. 
The 7th bar 'Were useful in helping me critically think about the factors' has 1 for Disagree, 2 for Neutral, 4 for Agree, and 5 for Strongly Agree.
Under this is plot C. A horizontal stacked-bar plot titled 'Provocations should.' 5 bars are present, with the label on the left part of the Y-axis. 
The 1st bar 'Identify shortcomings of the factor' has 1 for Neutral, 3 for Agree, and 8 for Strongly Agree. 
The 2nd bar 'Identify shortcomings of the provocation' has 4 for Neutral, 4 for Agree, and 4 for Strongly Agree. 
The 3rd bar 'Be Actionable' has 1 for Disagree, 4 for Neutral, 4 for Agree, and 3 for Strongly Agree. 
The 4th bar 'Be Relevant' has 3 for Agree, and 9 for Strongly Agree. 
The 5th bar 'Be supported by data in the dataset' has 2 for Strongly Disagree, 6 for Disagree, 3 for Agree, and 1 for Strongly Agree."

